Expert Selection in High-Dimensional Markov Decision Processes

In this work we present a multi-armed bandit framework for online expert selection in Markov decision processes and demonstrate its use in high-dimensional settings. Our method takes a set of candidate expert policies and switches between them to rapidly identify the best performing expert using a variant of the classical upper confidence bound algorithm, thus ensuring low regret in the overall performance of the system. This is useful in applications where several expert policies may be available, and one needs to be selected at run-time for the underlying environment.

==> experiments.tex <==
% !TEX root = 2017-CoRL.tex

All experiments were performed on a MacBook Pro 2013 with 2 GHz Intel Core i7 processors. The horizon $T$ for picking an expert was set to 100 environmental steps and all experiments were performed for a total of 1500 algorithm iterations. Each run of Algorithm \ref{alg:ucb} took approximately 12 minutes to run.  

In the Seaquest game, the goal is to eliminate as many sharks and enemy submarines as possible while rescuing divers, avoiding running out of oxygen and dodging incoming projectiles. In Section 5.1, we show the performance of the algorithm against the same set of occlusions used at training time. We then implement the algorithm on a set of new occlusions that the experts have not been trained on in Section 5.2. Lastly, we benchmark the algorithm against a set of baseline experts trained on random noise. In our implementation, all positive rewards from the environment (such as eliminating a shark or an enemy submarine) were normalized to one, and the rest to zero. Lastly, whenever an expert reaches the end of an episode after $k$ steps, where $k < T$, we reset the environment and let the expert run for the remaining $T-k$ steps.

\subsubsection{Expert Selection vs. Our Set of Occlusions}
\label{subsec:exp_sel_set_occl}

In our experiments, we used four different occlusions in the input to train each of the experts\footnote{The input images have dimensions of 84x84 pixels. The following list contains the 2D location of the upper left corner of the occlusion in the image, followed by the dimensions (height and width) of the occlusion itself: ~ O1:[10,30],[20,50] ~ O2:[25,10],[15,70] ~ O3:[42,10],[20,42] ~ O4:[10,10],[60,20]}. 
% \begin{figure}[!h]
% \centering
% \begin{subfigure}[b]{.2\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/occl_1}
%   \caption{Occlusion 1.}
% \end{subfigure}%
% \hfill
% \begin{subfigure}[b]{.2\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/occl_2}
%   \caption{Occlusion 2.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{.2\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/occl_3}
%   \caption{Occlusion 3.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{.2\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/occl_4}
%   \caption{Occlusion 4.}
% \end{subfigure}
% \caption{The above images correspond to the set of occlusions the experts were exposed to during training time. Each of the four experts was trained against only one of the occlusions.}
% \label{fig:occlusions}
% \end{figure}

\begin{figure}[t]
 \centering
 \includegraphics[width=0.8\columnwidth]{images/occlusion_figures.pdf}
 \caption{The above images correspond to the set of occlusions the experts were exposed to during training time. Each of the four experts was trained against only one of the occlusions.}
\label{fig:occlusions}
\end{figure}

The set of occlusions used at training time are shown in Fig. \ref{fig:occlusions} and were chosen to cover different areas of the image. Each occlusion  was used to train a single Q-network and each Q-network was included in our set of experts. Note that in Fig. \ref{fig:games_snapshot} the Seaquest domain looks different than in Fig. \ref{fig:occlusions}: this is due to the same preprocessing step on the raw images found in \cite{Minh_2013}.

The first test of the algorithm consists of running it against all the occlusions from our set. Since each expert was trained with a specific disturbance, we expect that given a fixed occlusion from our set, the corresponding expert will be chosen more often.

\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{plots/fig_train_occl2.png}
\caption{Each row shows the average over five runs of the algorithm using a fixed occlusion from our set. The first row corresponds to using occlusion one, the second row corresponds to using occlusion two and so on. The first column shows the iteration-normalized regret against the algorithm's iteration step. The second column shows the iteration-normalized number of calls to each expert against the algorithm's iteration step.}
\label{fig:alg_perf_k_occl}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{plots/fig_train_occl2.png}
\caption{Each row shows the average over five runs of the algorithm using a fixed occlusion from our set. The first row corresponds to using occlusion one, the second row corresponds to using occlusion two and so on. The first column shows the iteration-normalized regret against the algorithm's iteration step. The second column shows the iteration-normalized number of calls to each expert against the algorithm's iteration step.}
\label{fig:alg_perf_k_occl}
\end{figure}

Figure \ref{fig:alg_perf_k_occl} shows the performance of all experts for each of the four types of occlusions. As expected, given an occlusion from our set, the expert that was trained under that type of occlusion performed better than any of the other experts, thus getting picked more often. Moreover, we can also see that, as the algorithm proceeds, the iteration-normalized regret (the regret divided by the iteration number) converges to zero, meaning that the regret grows sub-linearly. 

It is important to note that in the second row, the rate at which the correct expert was picked was slower than the rest, even though the iteration-normalized regret also converged to zero. This behavior we believe might be caused by a mix of two factors: first, the generalization capabilities the Q-networks might have acquired at training time, and  second, the inherent performance differences between experts. In other words, while expert 2 was trained with occlusion two as shown in Fig. \ref{fig:occlusions}, expert 1 might have learned to generalize better to other occlusions, thus bringing its 100-step average reward to levels similar to expert 2. Another possible explanation is that since both experts had full image information for the bottom half of the screen, expert 1's performance might simply be significantly better than expert 2's when the submarine is in the lower half, thus making the 100-step average reward similar for both experts and making it difficult to distinguish which one of the two is better.

\subsubsection{Expert Selection vs. New Set of Occlusions}
\label{subsub:exp_sel_vs_new_occl}

An important aspect to take into account is that since our multi-armed bandit algorithm is agnostic to the input images, the types of occlusions we can use at run-time do not need to belong in our set. This is especially useful since it allows us to find the best-performing expert in our library of experts, which might happen to be comparable in performance to an expert that was specifically trained for that occlusion. Below, in Fig. \ref{fig:occlusions}, we show the new set of occlusions\footnote{The following list contains the 2D location of the upper left corner of the occlusion in the image, followed by the dimensions (height and width) of the occlusion itself: ~ O1:[50,10],[15,70] ~ O2:[10,50],[60,20] ~ O3:[40,20],[20,50] ~ O4:[10,15],[20,42]} and the corresponding performance of the algorithm.

% \begin{figure*}[!h]
% \centering
% \begin{subfigure}[b]{.2\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/un_occl1}
%   \caption{New occlusion 1.}
% \end{subfigure}%
% \hfill
% \begin{subfigure}[b]{.2\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/un_occl2}
%   \caption{New occlusion 2.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{.2\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/un_occl3}
%   \caption{New occlusion 3.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{.2\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{images/un_occl4}
%   \caption{New occlusion 4.}
% \end{subfigure}
% \caption{The above images correspond to a new set of occlusions the experts didn't experience at training time.}
% \label{fig:new_occlusions}
% \end{figure*}

% \begin{figure}[!h]
%  \centering
%  \includegraphics[width=0.95\columnwidth]{images/un_occlusions_figures.pdf}
%  \caption{The above images correspond to a new set of occlusions the experts didn't experience at training time.}
% \label{fig:new_occlusions}
% \end{figure}

Figure \ref{fig:alg_perf_unk_occl} shows that for most of the new occlusions, one expert was favored above the rest. For the new occlusions 1 and 3, the algorithm picked expert 3 more often than any other, and for occlusion four, the algorithm seemed to favor expert 1 more. An interesting aspect to note is that the experts that were picked more often are also the ones whose occlusions were most similar or had most overlap to the ones they were exposed to at training time. For occlusion 2, the algorithm did not seem to favor any one expert more than the rest within the first 1500 iterations. However, as expected, the two experts that were picked most often were the ones from our set with the highest 100-step average reward.

\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{plots/fig_new_occl}
\caption{Each row shows the average over five runs of the algorithm using a fixed occlusion from our set. The first row corresponds to using the new occlusion one, the second row corresponds to using the new occlusion two and so on. The first column shows the iteration-normalized cumulative reward against the algorithm's time step. The second column shows the iteration-normalized number of calls to each expert against the algorithm's iteration step.}
\label{fig:alg_perf_unk_occl}
\end{figure}

% \subsubsection{Expert Selection vs. Baseline Experts}

% As previously mentioned, a way to add robustness to disturbances is by adding corruptions to the training data. With this in mind, the  last experiment we perform is a comparison in performance between the algorithm and a set of three baseline experts trained with randomly changing occlusions\footnote{Every 10000 environment steps a new random occlusion appears replacing the previous one.}. In addition, we also show the performance of three experts trained without occlusions. 

% \begin{figure*}[!h]
% \centering
% \includegraphics[width=\textwidth]{plots/fig_bl_exp}
% \caption{Starting from the top left and going clockwise, each figure is associated with the (new) occlusion 1, 2, 4 and 3 respectively. Each figure depicts the iteration-normalized cumulative reward for the algorithm, as well as the iteration-normalized cumulative rewards for the agents trained with random occlusions and without occlusions.}
% \label{fig:alg_perf_vs_blexps}
% \end{figure*}

% Figure \ref{fig:alg_perf_vs_blexps} shows the iteration-normalized cumulative reward for the algorithm and the set of baseline experts. Except for the second new occlusion (top right plot in Fig \ref{fig:alg_perf_vs_blexps}), the algorithm performed better than both the experts with random occlusions and the experts with no occlusions in all cases. 

% It is important to emphasize that the performance of the algorithm is heavily dependent on our set of experts and their capacity to generalize. Therefore, it seems reasonable that the second new occlusion was the one where the performance was lowest, given that it was the most distinct one from our set of training occlusions.


